Intrinsic Mesh Simplification

This paper presents a novel simplification method for removing vertices from an intrinsic triangulation corresponding to extrinsic vertices lying on near-developable (i.e., with limited Gaussian curvature) and general surfaces. We greedily process all intrinsic vertices with an absolute Gaussian curvature below a user selected threshold. For each vertex, we repeatedly perform local intrinsic edge flips until the vertex reaches the desired valence (three for internal vertices or two for boundary vertices) such that removal of the vertex and incident edges can be locally performed in the intrinsic triangulation. Each removed vertex's intrinsic location is tracked via (intrinsic) barycentric coordinates that are updated to reflect changes in the intrinsic triangulation. We demonstrate the robustness and effectiveness of our method on the Thingi10k dataset and analyze the effect of the curvature threshold on the solutions of PDEs.

==> figures-spectral-cmp.tex <==
\begin{figure*}
    \centering
    \def\reswidth{0.22\linewidth}
    {
    \begin{tabular}{cccc}
    \includegraphics[width=\reswidth]{figures/spectral-cmp/bunny-intrinsic-1715-foot-dark.pdf} &
    \includegraphics[width=\reswidth]{figures/spectral-cmp/bunny-spectral-1715-foot-dark.pdf}  &
    \includegraphics[width=\reswidth]{figures/spectral-cmp/bunny-intrinsic-1715-hat-dark.pdf} &
    \includegraphics[width=\reswidth]{figures/spectral-cmp/bunny-spectral-1715-hat-dark.pdf}  \\
    Intrinsic Simplification (Ours) & Spectral Simplification &
    Intrinsic Simplification (Ours) & Spectral Simplification \\
    \includegraphics[width=\reswidth]{figures/spectral-cmp/frog-intrinsic-4e-2-nose.pdf} &
    \includegraphics[width=\reswidth]{figures/spectral-cmp/frog-qem-4440-nose.pdf} &
    \includegraphics[width=\reswidth]{figures/spectral-cmp/frog-intrinsic-4e-2-head.pdf} &
    \includegraphics[width=\reswidth]{figures/spectral-cmp/frog-qem-4440-head.pdf} \\
    Intrinsic Simplification (Ours) & QEM Simplification &
    Intrinsic Simplification (Ours) & QEM Simplification
    \end{tabular}
    }
    \caption{Solutions of a Poisson equations computed on simplified meshes
      obtained with Spectral Mesh Simplification and QEM. All solution are
      computed on the ``raw'' simplified mesh to better show the impact of
      simplification.}
    \label{fig:spectral}
\end{figure*}

